The End of a Myth: Distributed Transactions Can Scale

The common wisdom is that distributed transactions do not scale. But what if distributed transactions could be made scalable using the next generation of networks and a redesign of distributed databases? There would be no need for developers anymore to worry about co-partitioning schemes to achieve decent performance. Application development would become easier as data placement would no longer determine how scalable an application is. Hardware provisioning would be simplified as the system administrator can expect a linear scale-out when adding more machines rather than some complex sub-linear function, which is highly application specific. In this paper, we present the design of our novel scalable database system NAM-DB and show that distributed transactions with the very common Snapshot Isolation guarantee can indeed scale using the next generation of RDMA-enabled network technology without any inherent bottlenecks. Our experiments with the TPC-C benchmark show that our system scales linearly to over 6.5 million new-order (14.5 million total) distributed transactions per second on 56 machines.

==> a_response.tex <==
\section{Response for Paper \#267 (New: \#572)}

\noindent Dear Reviewers:

\noindent We would like to thank you for your highly constructive feedback on the paper.
As requested by the meta-reviewer, we added new experiments and clarified of the novelty of this paper over our own prior work.
Furthermore, we addressed all other issues as pointed out by the reviewers. 

\noindent In the following, we discuss the most important changes we made for this revision grouped by reviewer. The changes are highlighted in blue in the paper.\\

%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Reviewer 1}

\noindent\textit{\textbf{W1: Experimental section rather short, but sufficiently thorough at supporting claims.}}

\noindent\emph{Answer:}  We significantly extended our experimental evaluation in Section \ref{sec:evaluation}.
Most importantly, (1) we added a new experiment where we analyse the scalability of our new timestamp oracle and 
(2) measure the effect proposed optimizations from Section~\ref{sec:oracle:opti}. 
Furthermore, we compared the new timestamp oracle against the original timestamp oracle used in \cite{RDMAVision} (see Section \ref{sec:evaluation:exp4}) to show the improvement over our own prior-work. 

Secondly, we extended the experimental evaluation in Section \ref{sec:evaluation:exp2} where we vary the ratio of distributed transactions and included a comparison with H-Store, which represents a classical partition-based system using a shared-nothing architecture.
The goal was to show that (1) a redesign towards RDMA is needed to efficiently leverage fast networks and (2) partition-based systems are sensitive w.r.t. co-location and can not efficiently handle workloads that are hard to partition.
See also answers for D2 and D3 of Reviewer 2 for more details.
\\

\noindent\textit{\textbf{W2: Paper could be improved by having a short background/tutorial on one-sided/two-sided RDMA (for lazy readers).}}

\noindent\emph{Answer:} We agree that a background section on one-sided/two-sided RDMA would be helpful for the reader. 
However, because of space constraints we were not able to have a whole separate section but rather added further explanations to Section \ref{sec:architecture}.
For more explanations on RDMA and InfiniBand, we added text to refer readers to a more detailed reference. \\

\noindent\textit{\textbf{W3: Implementation details (i.e., the actual code) of NAM-DB not well covered. Is something available in open source?}}

\noindent\emph{Answer:}
%\erfan{I agree that we should make the code public to get more attention by becoming a good baseline for further details.}
This is an excellent point. We strongly believe in open-sourcing the system and having a long history of doing so (e.g., H-Store).
Not only do we think it is a good thing to do, but also we believe that it significantly raises the publicity of the work.  
However, we collaborate with Oracle on \system{} and they first need to grant us permission to make the code public.
Hopefully, that will happen in the next few weeks. 
\\

\noindent\textit{\textbf{D1: As described, the protocol seems to be doing single record RDMA operations. I wonder if batching updates might aid in reducing contention. This would like mean extending the APIs in the storage servers, which I'm not sure makes sense or is possible.}}

\noindent\emph{Answer:} One design principle in \system{} is to strictly separate compute and memory servers by using one-sided RDMA operations for remote data access.
This allows us to independently scale computation and memory and thus avoid that either of both resources becomes a bottleneck.
However, with the current generation of NICs, one-sided RDMA operations can not read/write data from/to multiple random memory locations in one roundtrip.
Therefore, batching is currently not possible with one-sided RDMA.
In future, with the next generations of RDMA NICs, this will most likely change and thus, batching might then become an interesting optimization that we can add to \system{}.
Furthermore, there exist also an interesting trade-off of when to use direct RDMA operations vs sending an RPC call to allow for batching. 
Again, studying this trade-off is beyond the scope of this paper. 
\\

\noindent\textit{\textbf{D2: I would have appreciated more discussion around your handling of variable-length records w.r.t. your fixed-length data formats. You suggest that the variable part can be stored elsewhere, but I didn't really get a good idea of how that was supported or what sort of impact variable-length records have on your performance.}}

\noindent\emph{Answer:} 
That is an excellent point and we did in fact evaluate different variable-length storage format but excluded the discussion from the paper because of space constraints.

Most importantly, we found that when using  RDMA, the latency for messages of up to $2$KB remains constant (i.e., shorter messages does not reduce latency) as shown in our vision paper \cite{RDMAVision}. 
Therefore, for many workloads it makes sense to store the data in a fixed-length memory region, including potential variable-length attributes and ``waste'' space for shorter values. 
We added this explanation to Section \ref{sec:memory:layout}.

If a variable-length record exceeds the $2$KB limit (as it is often the case with BLOBS), it is possible to include a pointer to an overflow region.
Accessing the overflow region, however, must then be implemented by using a separate network roundtrip that reads/writes the variable-length data using an additional one-sided RDMA read/write operation.
%As a small optimization in this design, it makes sense to store all fixed-length attributes in the beginning of the record and all variable-length records at the end to ensure that in most cases only the variable-length attributes ``flow over''.

We added some more details to Section \ref{sec:memory:layout}. 
\\

\noindent\textit{\textbf{D3: I also did not get a good understanding of how your indexes are maintained. The paper focuses on how the protocol behaves for transactions on the base data, and doesn't seem to mention updates to the secondary index structures.}}

\noindent\emph{Answer:} Indexes are stored in memory servers and updated within the boundaries of the transaction that also updates the corresponding table using RDMA operations  (i.e., we pay additional network roundtrips to update the indexes).
In case of a hash-index, updating is not different from a table which is basically implemented as a distributed hash table.
In case of a $B^+$-tree, we use two-sided operations that send the update information to the memory server, which then applies the index update and acknowledges the completion of the operation to the compute server.

In this paper, we use two-sided operations for updating a $B^+$-tree since a tree-like index would require multiple roundtrips between compute and memory servers when using one-sided operations and thus two-sided effectively reduces the latency.
However, in future we plan to look in hybrid update schemes for tree-like indexes that additionally use one-sided operations if the CPU of the memory server is becoming a bottleneck. 

For the revision, we added some more information about how index updates are executed within the transaction boundaries to Section~\ref{sec:compute:trans}. %\tim{we should put in some edits}
\\

\subsection{Reviewer 2}

\noindent\textit{\textbf{W1: The paper builds on top of the prior work and the differentiation is not fully clear.}}

\noindent\emph{Answer:} Please see the answer for D1.\\

\noindent\textit{\textbf{W2: Experimental evaluation does fully evaluate the claims made in the paper.}}

\noindent\emph{Answer:} Please see the answer for D2.\\

\noindent\textit{\textbf{W3: Comparison with partition-based approaches is missing.}}

\noindent\emph{Answer:} Please see the answer for D3.\\

\noindent\textit{\textbf{D1: It is very hard to differentiate this work from an earlier one [8], with the same authors. [8] made a case for OLTP databases as well and proposed RDMA-based SI protocol as well. The authors claim that the naive approach of [8] is "still not scalable" (though the previous paper claimed it was scalable) because: (i) RDMA operations to get unique timestamps have scalability issues, and (ii) it results in high abort rates. Unfortunately, neither of these two claims are verified experimentally. As a result, the motivation for this paper is not clear. Furthermore, the experimental evaluation does not show comparison with RDMA-based SI protocol in [8], leaving readers wonder how bad is the naive RSI anyways. In its current state, the contributions of the paper appear incremental and not fully differentiated.}}

\noindent\emph{Answer:} We have rewritten Section \ref{sec:intro:contrib} to better differentiate the contributions of this paper in the context of our vision paper \cite{RDMAVision}.

In our vision paper \cite{RDMAVision}, we only discussed a very initial prototype for distributed transaction processing to make the case why databases have to change in the presence of upcoming network technology. 
In fact, in the same paper we made also the case why OLAP systems have to change and explained and evaluated RDMA and Infiniband in detail. 
For the transactional part, we therefore made many simplifying assumptions (which we believe are fair for a vision paper but not a full submission like this one) regarding not only the storage management but also other central components.
For example, in \cite{RDMAVision} we have assumed that only the current (i.e., most recent) version of an attribute is stored in memory servers to simplify memory management and garbage collection. 
All transactions, which do require an older snapshot, have to abort. This prevents long-running reads, one of the main advantages of SI. 
Other differences are that we also neither had indexes, which limited the types of operations supported in the original prototype, nor used a logging scheme for recovery etc.
Furthermore, in \cite{RDMAVision} we only showed, as many other recent papers \cite{rdmajoin,flowjoin,highspeed}, the scalability of our prototype system in rather small deployments of up to $8$ nodes and the checkout transaction of the TPC-W benchmark, instead of having implemented the full TPC-C benchmark. 
Finally, we found that acquiring the timestamps is one of the main bottlenecks when scaling out beyond the 8 nodes; an important problem, which motivated this paper. 
Again, we believe that for a vision paper, which makes the case that the database architecture has to be reconsidered in the presence of new network technologies, these assumptions were reasonable. 

In contrast, in this paper we present the complete design of a truly scalable system that tackles all these limitations and supports complex transactional workloads.
One of the main contributions of this paper is the new scalable timestamp oracle, which is very different from the more classical design in \cite{RDMAVision} that used one globally-ordered counter.
Unfortunately, we could not directly compare the two systems on the large cluster, as the old system used libraries, which were not compatible with the OS on the large cluster (i.e. Oracle uses a proprietary Linux version). 
%\carsten{This is very shaky since we report driver versions in \cite{RDMAVision}  and in this paper which are actually the same. We should find a different argument.}
To still be able to compare the two systems, we therefore reimplemented the old timestamp oracle used in our vision paper \cite{RDMAVision} in our current \system{} system for this revision. 
This also enabled us to easily evaluate the old timestamp oracle with the full TPC-C benchmark which includes range queries.
While \system{} with the new oracle scales linearly up to 56 nodes as shown in Figure \ref{fig:exp1}, \system{} with the old oracle provides only a scalability up to 10 nodes and achieves a maximum throughput of approximately 0.5 million transactions per second.
We added this result at the end of Section \ref{sec:evaluation:exp1}.

When scaling out further, the throughput when using the old oracle in \system{} decreases to only 100.000 transactions per second on 56 nodes resulting from the contention on the old timestamp oracle; a similar effect that we see in the new scalability experiment for the timestamp oracle that we added to Section \ref{sec:evaluation:exp4}.
\\

%\begin{figure}
%\centering
%\vspace{-1ex}
%\includegraphics[width=0.75\columnwidth]{experiments/exp_oldvsnew.pdf}
%\vspace{-2.5ex}
%\caption{Initial Protoype vs. \system{}}
%\vspace{-4.5ex}
%\label{fig:app:exp1}
%\end{figure}



\noindent\textit{\textbf{D2: The experimental evaluation is not exhaustive; the paper proposes a system which describes several ideas but none of them are evaluated in detail, e.g., the effectiveness of scalable timestamp generation is not shown; likewise 4.2 shows further optimizations to the timestamp oracle but their impact is not measured. A more exhaustive evaluation of different aspects of the system is much desired.}}

\noindent\emph{Answer:} We added a new experiment to separately analyze the scalability of our new timestamp oracle as well as the benefits of the various oracle optimizations  (see Section \ref{sec:evaluation:exp4}).

As a baseline in this new experiment, we used the original timestamp oracle of our vision paper \cite{RDMAVision}.
This timestamp oracle implements a classical design with one globally-ordered counter \cite{saphana}, which is accessed concurrently via RDMA operations from different compute server threads as described in Section \ref{sec:protocol}. 
To analyze the impact of the different optimizations discussed in Section \ref{sec:oracle}, we evaluated them in isolation (e.g., we turned one optimization after another on) using the same scale-out experiment. 

The results of this experiment show that the original oracle could sustain the load generated by our initial prototype of the vision paper that achieved $1.1M$ transactions per second in a cluster of $8$ nodes.
Different from the original oracle, however, our new oracle is able to scale to much larger deployments.
In fact, in its basic version without any additional optimizations the oracle on a single machine can already sustain a load of up to $20M$ timestamp operations; that is, for our experiments the cluster could almost be twice as big before our timestamp oracle w/o any additional optimizations becomes a bottleneck 
(note, it is ``only'' twice as big, as TPC-C  reports only the new-order transactions, which represent $45\%$ of the transactions). 
With all optimizations enabled, the timestamp oracle scales to  $135M$ timestamp operations on a single machine and thus would support even much much larger deployments.\\

\noindent\textit{\textbf{D3: While eliminating the requirement for co-location as in earlier distributed systems is nice, I wonder how bad are the partition-based approaches anyways; do they really get partition so wrong in most cases? An experimental comparison with prior state of the art partitioning could really help answer this question.}}

\noindent\emph{Answer:}  We added another baseline, comparing NAM-DB with H-Store \cite{Andy-thesis} to our experimental evaluation in Section \ref{sec:evaluation:exp2} to show how well a classical partition-based system behaves when we vary the ratio of distributed new-order transactions from $0\%$ to $100\%$ in the TPC-C benchmark.
We choose H-Store as it is one of the few freely available distributed in-memory transactional database systems with a classical shared-nothing architecture.

In this experiment, we executed the distributed version of H-Store without any modifications over InfiniBand (IB) using IP over IB as communication stack.
As a main result, we found out that H-Store has an overall much lower throughput than \system{}.
When the database is perfectly partitionable and we thus have $0\%$ distributed transactions (i.e., there are no distributed transactions required at all) we only reach $11$K transactions per second.
First, we were surprised by the low throughput. Thus, given the H-Store expertise in our group we tuned the system further. 
However, it turns out that these numbers are in fact in line with the ones reported in various research papers (e.g., \cite{HStore:SIGMOD:2012}).
Though the important take-away of the experiment is not that \system{} achieves a higher throughput, but that at $100\%$ distributed transactions the throughput of H-Store drops $90\%$, to only $900$ transactions per second, while our system still achieves more than $1.5M$ transactions under the same workload; a small performance drop compared to its no-distributed-transaction case.
This clearly shows the sensitivity of the shared-nothing design for data-locality.

Figure \ref{fig:exp0a} shows the results of this experiment. We have added these results to the text of Section \ref{sec:evaluation:exp2}.
However, we did not add the additional line for H-Store to Figure \ref{fig:exp3a} in the paper since it would not have been really visible for the given y-scale. Below, we therefore added Figure \ref{fig:exp0b} to show the throughput of H-Store in a separate plot.
However, we omitted the additional plot (H-Store only) in Figure \ref{fig:exp0b} from the paper because of space constraints.

\begin{figure}[ht]
\centering
\subfigure[All Systems]{
   \includegraphics[trim=5 0 20 0,clip,width=.46\columnwidth]{experiments/exp0_hstore.pdf}
   \label{fig:exp0a}
}
 \subfigure[H-Store only]{
   \includegraphics[trim=5 0 20 0,clip,width=.46\columnwidth]{experiments/exp0_hstore_isolated.pdf}
   \label{fig:exp0b}
}
\vspace{-3.5ex}
\caption{Throughput of \system{} vs. H-Store}
\end{figure}

\noindent\textit{\textbf{D4: Finally, while the InfiniBand based approaches win in terms of performance, how do the costs compare with traditional commodity hardware? Also, how do Ethernet based RDMA, such as RDMA over Converged Ethernet (RoCE), compare with the propsed InifinBand architecture? It would be nice to have a clarification on how much of the performance is due to InfiniBand and RDMA respectively.}}

\noindent\emph{Answer:} InfiniBand is becoming increasingly affordable. 
For example, a small cluster with eight servers, each with two Xeon E5v2 CPUs and one 2-port InfiniBand FDR 4$\times$ NIC, and a total of 2TB of DDR3-1600 memory costs under \$80K, with the InfiniBand switch and NICs representing roughly \$20K of the total cost.
This is comparable to the cost of more traditional Ethernet-based networking hardware for such a cluster.

Moreover, there also exist other network technologies that support RDMA and thus avoid the high overhead of the TCP/IP stack.
One example is RoCE which provides RDMA over converged Ethernet.
However, regarding the performance, RoCE over 40Gpbs Ethernet still has $2\times$ higher latencies than InfiniBand FDR \cite{ibvsroce}.
Another interesting option in future will be Intel's OmniPath architecture, which also includes RDMA and promises even lower latencies than InfiniBand at a comparable bandwidth.

We believe that the scalable design of \system{} can be used on all these technologies.
In fact, we will soon get access to a $256$ node OmniPath cluster.
Analyzing \system{} on this hardware is an interesting future avenue of work.\\

\subsection{Reviewer 3}

\noindent\textit{\textbf{W1: Low performance. Some modern systems achieve 2+x of the perf only on a single (beefy) 16-socket machine vs 56 2-socket nodes.}}

\noindent\emph{Answer:} Please see the answer for D1.\\

\noindent\textit{\textbf{W2: Ignored related work.}}

\noindent\emph{Answer:} Please see the answer for D2.\\

\noindent\textit{\textbf{D1: The overall approach is quite innovative. But there is some concern on the performance of the system. The authors say that they achieve 6.5M distributed NewOrder transactions per sec on 56 machines (or 3.6M TPS without locality optimizations) in TPC-C. Modern memory-optimized OLTP systems, such as Silo (SOSP'13) and ERMIA (SIGMOD'16), achieve somewhere in the order of 0.5M  TPC-C transactions per second, on a single commodity node.
Even worse, let's take for example a paper from HP Labs that was recently accepted at VLDB'17. This paper presents two systems that get 17Mtps on a single beefy (16 sockets) node when running TPC-C. So, one 16-socket node (16 Xeons) gets 2+x higher throughput than 56 2-socket nodes (116 Xeons). It would be interesting if the authors at least commented on this issue.}}

\noindent\emph{Answer:} 
Thanks for pointing us to the HP-paper. At a first glance we were very surprised by the high throughput they are able to achieve. 
However, the results look quite differently if one puts them into the right perspective. 

(1) First, for our evaluation we follow the TPC-C specification and only report the new-order transaction for the total throughput (6.5Mtps), whereas the authors of the HP-paper count every transaction to get to the 17Mtps. 
Unfortunately, the authors did NOT clearly mention that in the paper, but we got in touch with them and they confirmed that they count every transaction. 
Counting all transactions, we actually achieve $\approx 14.5$Mtps.

(2) Still, even with counting every transaction the throughput per core is roughly 4x lower in our system; $17Mtps /$ $288  cores$ $\approx 59Ktps/core$ 
(HP with 16 sockets, each having 18 cores) vs $14.5Mtps / 896 cores \approx 16.8 Ktps/core$ (our system on cluster A with 56 nodes two sockets per machine, each with 8 cores).
However, we know from our experiments that we are network-bandwidth bound, which is roughly $1/4$ of the main-memory bandwidth. 
To that end, we speculate that if we were able to increase the network-bandwidth by a factor of $4$, our system would actually be able to achieve the same throughput as the very beefy HP machine. 
In our vision paper \cite{RDMAVision}, we already showed that it is possible to achieve the same network bandwidth as the main-memory bandwidth by having 4 FDR NICs per dual-socket machine. 
Furthermore, according to the current IB specification, in the future just one dual-port HDR NIC would be able to achieve the same result (of course assuming that the main-memory bandwidth is not significantly increasing anymore). 

However, in contrast to the beefy HP machine, with our approach the user would be able to slowly scale-out the cluster based on the demand 
and would be able to scale even beyond the 17Mtps; at least we know from our experiments that our timestamp oracle would be able to sustain the load and we are not aware of any other bottlenecks.
Furthermore, our locality-aware deployment is not yet as highly optimized as the one in \cite{hpwork} (e.g., all local request still go through the NIC instead of bypassing it) as it was not the focus of this paper. 
Finally, \cite{hpwork} implements MOCC, a variant of OCC and not SI. 
As with most OCC implementations, they rely on a (re-)validation of the read and write set, which performs very poorly for long running read transactions as it either blocks other transactions (when using locks as MOCC does for hot items) or the long running transactions always get aborted. 
In contrast, SI is ideal for long-running reads and thus, it is especially good for the new trend towards having mixed transactional and analytical workloads.

Thanks again for pointing us to the HP publication; after all, we were pleased to find out how our system compares to the state-of-the-art in scale-up approaches. 

%Moreover, at the moment \system{} is network-bound since we only have one NIC per machine whereas in order to match the memory-bandwidth we would require two NICs per socket (i.e., four NICs per machine) as shown in \cite{RDMAVision}.
%Taking both factors into account, we speculate that the throughput in \system{} on the 56 node cluster when counting all transactions (and not only new-order transactions) and using four NICs per machine would be 6.5Mtps * 100/45 * 4 $\approx$ 58Mtps.
%This is equivalent to 65Ktps per core (since cluster $A$ has in total 896 cores).
%Compared to the paper mentioned before from HP Labs which uses a 16 socket machine with 288 cores in total, the per core throughput is very similar with 60Ktps.
%\\

\noindent\textit{\textbf{D2: There are a lot of studies/related work that it is being ignored/not mentioned. For example, there is a lot of work by Bailis on distributed transaction processing and by Porobic on transaction processing "Islands" that seem to be quite related.}}

\noindent\emph{Answer:} We have extended the related work section. \\

